Quantum Combine and Conquer and Its Applications to Sublinear Quantum Convex Hull and Maxima Set Construction

We introduce a quantum algorithm design paradigm called combine and conquer, which is a quantum version of the "marriage-before-conquest" technique of Kirkpatrick and Seidel. In a quantum combine-and-conquer algorithm, one performs the essential computation of the combine step of a quantum divide-and-conquer algorithm prior to the conquer step while avoiding recursion. This model is better suited for the quantum setting, due to its non-recursive nature. We show the utility of this approach by providing quantum algorithms for 2D maxima set and convex hull problems for sorted point sets running in $\tilde{O}(\sqrt{nh})$ time, w.h.p., where $h$ is the size of the output.

==> algorithm.tex <==
\section{Algorithm}

\newpage 
\subsection{Maxima Set}

Assume set is sorted, split into sqrt(n) sized blocks, report the max y coordinate in each block. 

Split into h blocks with size sqrt(n/h). Each block will be labeled with an integer $j$, and will also carry $O(h)$ ancilla qubits. More concretely, each block will have the form 
\begin{equation}
\ket{S_j}\ket{0}_{I_t^j}\ket{0}_{p_{I_t^j}}\ket{0}_{I_r^j}\ket{0}_{p_{I_r^j}}\ket{0}_{I_1^j}\ket{0}_{p_{I_1^j}}\cdots \ket{0}_{I_h^j}\ket{0}_{p_{I_h^j}}\ket{0}_{\text{count}^j},
\end{equation}
where 
\begin{itemize}
    \item $I_t^j$ stores the index of the tallest point in block $j$, 
    \item $I_r^j$ stores the index of the tallest point in all the blocks to the right of block $j$, 
    \item $I_i^j$ for $1 \leq i \leq h$ will store the indices of upto $h$ potential maxima points found in block $j$, 
    \item $p_{I}$ is the $x$ and $y$ coordinate of the element with index $I$, and
    \item the count$^j$ register records how many maxima points have been found throughout the algorithm in block $j$.
\end{itemize}

Given the registers block separated in the above form, the algorithm proceeds as follows. 

\begin{algorithm}
\caption{Maxima Set($S$)}\label{alg:maxima-set-info}
\begin{algorithmic}[1]
\Require $S$ is sorted in lexicographic order, and can be accessed by a data loading unitary. 
\State Let $\ket{S_0, S_1, \ldots, S_{h-1}}$ be $S$ subdivided into $h$ separate $O(n/h)$ sized blocks. 
\State (*) Load each of the registers $S_j$ into a QRAM state, $\ket{\psi_j}$. 
\State For each $\ket{\psi_j}$, run maximum finding over the $y$ coordinates of the points. Store the index and coordinate information in registers $I_t^j$. 
\For{j from $h - 1$ to 1}
\If {$p_{I_t^j}$.y $< p_{I_t^{j + 1}}$.y } 
    \State $I_r^j = I_t^j$
\Else 
\State $I_r^j = I_r^{j+1}$
\EndIf
\EndFor     
\If{count$^j = 0$ } % count is zero, input = t, else input = I_count
\State $I_s = I_t^j$
\Else
\State $I_s = I_{\text{count}^j}$
\EndIf 
\While{True}
\State \textbf{Search}($I_s$, $I_r^j$)
\If{there are no more viable solutions, }
\State \textbf{break}
\Else 
\State count$^j$++
\State Store the search result in $I_{\text{count}^j}$
\EndIf
\EndWhile
\State Check each of the $h$ blocks, and output \text{count}$^j$ many solutions stored.
\end{algorithmic}
\end{algorithm}



\begin{algorithm}
\caption{Search($I_s$, $I_f$)}\label{alg:q-search}
\begin{algorithmic}[1]
\Require We assume that $I_s$ and $I_f$ are passed along with the data values at the indices.    
\If{$I_s < I_f$}
\State Return 0
\Else
\State Run maximum finding subject to the function 
\begin{equation*}
    f(I) = \begin{cases}
        1 & \text{if $I_s \leq I \leq I_f$} \\ 
        0 & \text{otherwise.}
    \end{cases}
\end{equation*}
\EndIf
\end{algorithmic}
\end{algorithm}


\subsubsection{Runtime}

The runtime of algorithm \ref{alg:maxima-set-info} is $\tilde{O}(\sqrt{nh})$. 

Using the data loading construction from \cite{cortese2018}, the data loading unitary can be applied using $O(\log n)$ time. 
% For simplicity, assume that $h$ is a power of 2. Then to load block $S_j$, we set the first $\log_2 h$ bits of the index register to $j$, and then apply Hadamard gates to all lower order qubits. 
This achieves a superposition state 
\begin{equation}
    \sum_{i = 0}^{n/h - 1} \ket{i}\ket{p_i}.
\end{equation}
Line 3 takes $\overset{\sim}{O}(\sqrt{n/h})$ time. 
The loop starting at line 4 takes $O(h)$ time. 
The loop at line 16 takes $\overset{\sim}{O}(\sqrt{nh})$. 
Finally, line 25 takes $O(h)$ time. 




\subsection{Maxima Set}

% We assume that the input is given in the form $\ket{p_1 p_2 \cdots p_n}$, where $p_i$ is a pair of $x$ and $y$ coordinates. 

% We will partition this input register into $\sqrt{n}$ subregisters $\ket{S_1}, \ket{S_2}, \ldots, \ket{S_{\sqrt{n}}}$.

% For each input element $p_i$, we will also attach $\log_2 n$ ancilla regiters, each with one qubit, to store data throughout the computation. The ancilla qubit $M_k$ will record whether $p_i$ is a maxima point in the subset at the current level. These registers can be computed in a bottom up fashion with calls to two unitaries at each level. 

% Consider a tree with $n$ leaves, each corresponding to one of the input elements. We will group elements together if they are in the same subtree rooted at depth $k$. The value in register $M_k^i$ will be $\ket{1}_{M_k^i}$ if it is a maxima point in the subset associated with the subtree rooted at depth $k$, and $\ket{0}_{M_k^i}$ otherwise. This can be computed using two unitaries that encode the following two boolean functions. First, we will have a function $f: (\mathbb{Z} \times \mathbb{Z})^2 \rightarrow \{0, 1\}$ such that 
% \begin{equation*}
%     f(p_i, p_j) = \begin{cases}
%         1 & \text{if $p_i$ is dominated by $p_j$} \\
%         0 & \text{otherwise.}
%     \end{cases}
% \end{equation*}
% The second function $g: \{0, 1\}^2 \rightarrow \{0, 1\}$ is used to combine information from computing $f$ along with the previous data stored with each point. 
% \begin{equation*}
%     g(b_f, b_p) = \begin{cases}
%         1 & \text{if this point was dominating at the previous level, and not dominated.} \\
%         0 & \text{otherwise. }
%     \end{cases}
% \end{equation*}


% Actually this approach may not work. In the worst case, we will have each subregister storing $O(\sqrt{n})$ candidates for the maxima set, but the last register has points that dominate every other point, meaning we need to do $O(\sqrt{n}\cdot \sqrt{n})$ work to combine the solutions, even though the output has some constant $h$ points which happen to be in the final register. 

% \subsection{Maxima Set}

% \textbf{On a non D+C algorithm}
% When not using any divide and conquer approach, this problem boils down to implementing a coherent unitary that applies the function 
% \begin{equation}
%     f(j) = \begin{cases}
%         1 & \text{ if $p_j$ is in the maxima set, and } \\
%         0 & \text{ otherwise.}
%     \end{cases}
% \end{equation}
% We then apply this unitary to the superposition of indices, then sample to find all $h$ points in the maxima set. The amplitude amplification can be done in $O(\sqrt{n/h})$ time, and we need $\overset{\sim}{O}(h)$ samples to retrieve all $h$ points with high probability. This gives a final runtime of $\overset{\sim}{O}(\sqrt{nh}T)$ where $T$ is the time complexity of the unitary $U_{in}$. It is not immediately clear how to implement $T$ in a coherent way. Comparing against every other point in $P$ will require $O(n)$ gates. 

% \;

% \textbf{Challenges with median finding}
% The existing median finding algorithm finds subsets with size $(1 + \epsilon)N/2$ in time $O(\frac{1}{\epsilon}\log\frac{1}{\epsilon}\log\log \frac{1}{\epsilon})$ w.h.p. It also is not amenable to run coherently, as it requires sampling to reconstruct the median. If we run a divide and conquer type algorithm, we eventually need to find $O(N)$ different medians. 

% Furthermore, if we have a QRAM type register storing all the points, we eventually need to have $O(N)$ different medians stored somehow using at most $O(\log{N})$ calls to the algorithm. The number of states in superposition does not shrink in the subsequent calls, so our approximation factor does not scale with the actual number of points we are interested in. We \textit{could} run $n$ different calls to $k$-th largest element separately, but this may be hard to parallelize. 

% \;

% This may motivate some interest in finding a coherent algorithm to find the median? This is also a classic divide and conquer problem, so a non-sampling algorithm could be interesting.

% \; 

% % QRAM Attempt Sorted version
% We begin with an algorithm that receives the input via access to a black box function $P$, which takes as input an index $i$ and returns the $i$-th point $p_i$. In this initial attempt, we further assume that the inputs are encoded in the black box in sorted order, that is, $p_i \leq_L p_j$ iff $i < j$. This allows us to prepare the state $\sum_i \ket{i}\ket{p_i}$. We can parallelize our access to this function, and create multiple copies of the state with time equivalent to a single query. 
% % Would be nice to name this model to distinguish it from sequential input. 

% % A unitary that directly takes two registers of the input and compares each point against the other points would require Omega(n) samples... The register that stores the relation of a pair is a superposition of n^2 states, if there is only a single pair that returns YES, this is 1/n^2 amplitude. 

% % Doing this by matching number of bits reduces this to a superposition of n states. 


% - Find the lexicographic maximum element that is unmarked. Output this element. 
% - Mark all elements dominated by or equal to this element. 
% - End when all elements have been marked.
% => $O(h\sqrt{n})$


% % Split into sqrt(n) sized blocks. In each block find the largest point lexicographically and return. 
% % Now take each pair of blocks and use the information to 
% f(i) = 



% Maxima set algorithm where the items in $S$ are sorted in lexicographic order, and the number of points $h$ is known in advance. 
% \begin{algorithm}
% \caption{Maxima Set($S$)}\label{alg:maxima-set}
% \begin{algorithmic}[1]
% \Require $S$ is sorted in lexicographic order, and given as a list $\ket{x_1, x_2, \ldots, x_n}$ stored sequentially. 
% \State Let $\ket{S_1, S_2, \ldots, S_{\sqrt{h}}}$ be $S$ subdivided into $h$ separate $O(n/h)$ sized blocks. 
% \State Load each of the registers $S_i$ into a QRAM state, $\ket{\psi_i}$. 
% \State For each $\ket{\psi_i}$, run maximum finding over the $y$ coordinates of the points. Record the index of the point that achieved this max. 
% \State Using the $h$ maximums, 

% \State Recursively call minimum finding on each of the blocks. Store the outputs in the data register $D$ $\ket{\min(S_1), \ldots, \min(S_{\sqrt{n}})}_D$
% \State Load each block $i$ of the output register into an indexed superposition, $\frac{1}{n^{1/4}}\sum_{j=1}^{\sqrt{n}}\ket{j}_{I_i}\ket{x_{i, j}}_{D_i}$
% \State Run the minimum finding algorithm on register $D_i$, storing the result in the output register.
% \end{algorithmic}
% \end{algorithm}


% What if we know h in advance? Timothy Chan Jarvis march algorithm based on this knowledge. 

% Given point set S and query point x, return YES/NO if x is in Conv(S), and if YES, return the smallest triangle in S that contains x. 

% Support vector problem: Return the line that separates two sets R and B. 


